Symmetries and Correlations in Strongly Interacting One-dimensional Quantum Gases

The main focus of this thesis is the theoretical study of strongly interacting quantum mixtures confined in one dimension and subjected to a harmonic external potential. Such strongly correlated systems can be realized and tested in ultracold atoms experiments. Their non-trivial permutational symmetry properties are investigated, as well as their interplay with correlations. Exploiting an exact solution at strong interactions, we extract general correlation properties encoded in the one-body density matrix and in the associated momentum distributions, in fermionic and Bose-Fermi mixtures. In particular, we obtain substantial results about the short-range behavior, and therefore the high-momentum tails, which display typical $k^{-4}$ laws. The weights of these tails, denoted as Tan's contacts, are related to numerous thermodynamic properties of the systems such as the two-body correlations, the derivative of the energy with respect to the one-dimensional scattering length, or the static structure factor. We show that these universal Tan's contacts also allow to characterize the spatial symmetry of the systems, and therefore is a deep connection between correlations and symmetries. Besides, the exchange symmetry is extracted using a group theory method, namely the class-sum method, which comes originally from nuclear physics. Moreover, we show that these systems follow a generalized version of the famous Lieb-Mattis theorem. Wishing to make our results as experimentally relevant as possible, we derive scaling laws for Tan's contact as a function of the interaction, temperature and transverse confinement. These laws display interesting effects related to strong correlations and dimensionality.

==> ExpCorr.tex <==
\chapter{Dispositifs expérimentaux pour mesurer des fonctions de corrléation de l'intensité}\label{Chap:ExpCorr}

\minitoc\newpage

  \section{Différents montages expérimentaux pour la mesure des corrélations d'intensité}\label{Sec:SetUpCorr}
  
    \subsection{Mesures homodynes}\label{Subsec:Homodyn}
    
      \subsubsection{Expériences de Handurry Brown et Twiss}\label{Subsubsec:HBT}
      
Expérience historique de HBT avec la mesure du diamètre angulaire des étoiles. HBT avec des photons.

      \subsubsection{Homodynage et atomes froids}\label{Subsubsec:HomodynAF}
    
Mesures homodynes avec les atomes froids. Domaine spectral (auto battement) \cite{Article:Jurczak1995} et temporel \cite{Nakayama2010} et
Bali.

    \subsection{Mesures hétérodynes}\label{Subsec:Heterodyn}
    
Principe de la mesure hétérodyne avec le battement avec un oscillateur local. Exemple avec \cite{Article:Westbrook1990}.

  \section{Piégeage et caractérisation d'une vapeur atomique froide}\label{Sec:PrepMOT}

Dans le cadre de cette thèse, nous cherchons à étudier la diffusion de la lumière, éventuellement en présence de gain, à l'intérieur
d'une vapeur de rubidium refroidie à quelques centaines de micro Kelvin. Pour cela, nous utilisons un piège magnéto-optique
(abrégé par MOT pour \emph{magneto-optical trap} dans la suite). Son principe a été proposé par Jean Dalibard dans les années 80,
puis réalisé expérimentalement quelques années après \cite{Raab1987}. De nos jours, le MOT est à la base de la majorité des
expériences d'atomes froids.

Son principe de fonctionnement est basé sur deux ingrédients : une force de dissipation, visant à ralentir les atomes et
à les refroidir, et une force de rappel, utilisée pour les maintenir proche du centre du piège. La force de dissipation est
générée par trois paires de faisceaux contra-propageant orientées selon les trois directions de l'espace et désaccordés vers le
rouge (fréquence du laser inférieure à la fréquence de résonance atomique considérée), dont les polarisations sont circulaires
opposées. Étudions le cas uni-dimensionnel. On considère un atome animé d'une vitesse positive dirigée selon la direction
$\vecteur{\hat{x}}$. Ainsi, en tenant compte de l'effet Doppler, le laser se propageant selon $-\vecteur{\hat{x}}$ verra sa
fréquence se décaler vers la résonance atomique. Il est donc diffusé plus efficacement par l'atome, et lui transfère une certaine
quantité de mouvement. C'est le principe de la pression de radiation et du refroidissement Doppler. De ce fait, le laser
colinéaire à la vitesse de l'atome a sa fréquence qui s'éloigne de la résonance atomique et interagit moins efficacement avec
l'atome. La force finale tend donc à ralentir les atomes, indépendamment de leur position. Enfin, la force de rappel
supplémentaire, nécessaire au piègeage des atomes, est obtenue grâce à un gradient de champ magnétique, généré par une paire de
bobines en configuation anti-Helmholtz. Le principe de fonctionnement du MOT est résumé sur la figure~\ref{fig:PrincipeMOT}. La
physique des pièges magnéto-optique ne sera pas plus évoquée ici, le lecteur pouvant se référer à la littérature abondante traitant
de ce sujet, voir \cite{Autre:Dalibard} pour une introduction.


\begin{figure}\centering
\input{/home/aurelien/These/Recherche/Manuscript/ExpCorr/TiKZ/PrincipeMOT.pgf}
  \caption{Schéma de principe d'un piège magnéto-optique. Une paire de bobines en configuation anti-Helmholtz génère un gradient
  de champ magnétique tri-dimensionnel. Il permet la levée de dégénérescence des niveaux ayant un moment cinétique non nul, en
  particulier le niveau excité $\ket{F^{\prime} = 1}$. Les lasers utilisés pour le refroidissement sont désacordés vers le rouge,
  désaccord négatif, et ont des polarisations circulaires croisées. Un seul laser ne peut induire une transition que vers un
  sous-niveaux Zeeman particulier du niveau excité, suivant les règles de sélection. A chaque fois qu'un atome s'éloigne de la
  région du centre du piège, où le gradient est nul, la fréquence de la transition vers un des sous-niveaux est diminuée par effet
  Zeeman. Le laser correspondant est donc quasi-résonant et tend à ramener l'atome vers le centre du piège. Précisons que, dans le
  cas de la présence de plusieurs niveaux stables, un repompeur (non montré sur la figure) est nécessaire pour maintenir tous les
  atomes dans l'état utilisé pour le refroidissement.}
    \label{fig:PrincipeMOT}
\end{figure}

    \subsection{Préparation d'un piége magnéto-optique}\label{Subsec:MOT}

La spécificité du groupes Atomes froids à Nice réside dans l'étude de MOT avec un grand nombre d'atomes. Pour arriver à capter
beaucoup d'atomes dans ce type de pièges, il est nécessaire d'avoir à disposition plusieurs éléments. Tout d'abord, une source
laser est requise pour permettre le refroidissement, dont la fréquence peut être ajustée finement autour de la résonance atomique
avec une précision de l'ordre de la largeur naturelle de l'état excité considéré et dont la polarisation doit être finement
contrôlée. Ensuite, des bobines sont nécessaires pour créer le gradient de champ magnétique obligatoire pour le piègeage des
atomes. Finalement, le piége doit être réalisé dans une enceinte à vide de sorte à isoler l'élèment chimique piégé de toute autre
corps capable d'entraîner une relaxation par collisions. Le schéma~\ref{Fig:EnsembleManip} résume ces différents éléments
nécessaires à la résalisation d'un MOT.

\begin{figure}\centering
 \input{/home/aurelien/These/Recherche/Manuscript/ExpCorr/TiKZ/SchemaManip.pgf}
  \caption{Schéma global de l'expérience, rerésentant les différents éléments nécessaires au bon fonctionnement d'une expérience
  d'atomes froids.\textcolor{red}{RAJOUTER LES FLECHES DES FAISCEAUX MOT ET POMPE}}
    \label{Fig:EnsembleManip}
\end{figure}

Depuis le montage de l'expérience au cours des années 1990, plusieurs modifications ont été apportées pour la stabiliser. Néamoins,
l'architechture reste la même. Dans ce paragraphe, nous présentons les principaux éléments pour la réalisation pratique d'un piége
magnéto-optique de \Rb, en utilisant la transition fermée $\ket{F = 3} \to \ket{F^{\prime} = 4}$ de la raie D2 du rubidium,
caractérisée par la largeur $\Gamma$ de l'état excité donnée par $\Gamma/2\pi = \unit{6.066}{\mega\hertz}$. De plus amples détails
pourront être trouvés dans les manuscripts de thèse de Quentin Baudouin \cite{Baudouin2014b} et Samir Vartabi-Kashanian
\cite{Kashanian2016}.

      \subsubsection{Système à vide}\label{Subsubsec:Vide}
  
Dans notre expérience, le MOT est chargé directement à partir d'une vapeur de \Rb~à température ambiante. Il est possible d'adapter
la quantité de vapeur présente dans l'enceinte à vide depuis une source de rubidim. Cela fait donc varier la pression de rubidium à
partir de laquelle le MOT est chargé. Nous reviendrons plus tard sur l'influence la pression résiduelle sur le MOT. La  pression
typique requise pour le bon fonctionnement de l'expérience est de $\unit{\power{10}{-8}}{\milli\bbar}$. Les atomes sont chargés
dans une cellule de quartz cubique de largeur $\unit{10}{\centi\meter}$. Cette cellule est sans armature métallique, ce qui permet un
très large accès optique.

Au quotidien, le vide est assuré par une pompe ionique Varian Starcell Valcon Plus 40 ($\unit{34}{\liter\per\second}$), installée
au cours de cette thèse. Elle est pilotée par un contrôleur MiniVac Controller. L'estimation de la pression s'effectue soit par la
mesure du courant circulant dans la pompe ionique, soit par une jauge de pression située à proximité de la pompe à vide. Nous
verrons à la section~\ref{Subsubsec:Loading} comment avoir une mesure de la pression ambiante en utilisant le MOT en lui-même.

      \subsubsection{Champ magnétique}\label{Subsubsec:ChampB}

Le gradient de champ magnétique requis pour la création de la force de rappel pour le piégeage des atomes est obtenu par deux bobines
en configuration anti-Helmholtz, permettant d'obtenir une champ quadrupolaire non uniforme. Ce champ est nul au centre du piège et
augmente en intensité avec la distance. Un gradient de champ magnétique de l'ordre de $\unit{10}{\gauss\cdot\centi\reciprocal\meter}$
est ainsi généré. Pour compenser les champs magnétiques parasites, en particulier celui terrestre, trois paires de bobines en
configuration Helmholtz sont ajoutées. Enfin, un blindage magnétique entoure la pompe pour s'affranchir d'éventuels gradients
supplémentaires générés par ses aimants. \textcolor{red}{Rajouter les détails de la coupure du champ et sa vitesse.}

      \subsubsection{Configuration laser pour le piégeage d'atomes froids}\label{Subsubsec:Lasers}
 
Plusieurs sources lasers sont requises dans une expérience d'atomes frois, que ce soit pour piéger les atomes, les sonder ou les
pomper. Tous ces lasers sont à une longueur d'onde proche de $\unit{780}{\nano\meter}$, sur la raie D2 du rubidium 85. Nous détaillons
dans cette section les lasers utilisés ainsi que les systèmes d'asservissement en fréquence.
 
	\paragraph{Système laser}\label{Parag:Lasers}
  
Trois sources lasers sont utilisées sur notre montage expérimental~: une en étant que référence de fréquence, une pour piéger et
refroidir effectivement les atomes et une dernière pour maintenir les atomes dans le piége.

Premièrement, une diode DBR (Distributed Bragg Reflector, Yokogawa YL78XN), de puissance nominale $\unit{5}{\milli\watt}$ et de
largeur $\unit{2}{\mega\hertz}$, est utilisée en tant que laser maître. Elle est asservie par absorption saturée sur le cross-over 
$\ket{F = 2} \to \ket{F^{\prime} = 2}/\ket{F = 2} \to \ket{F^{\prime} = 3}$ du \RbIso. Par ailleurs, une diode DFB (Distributed
Feebdack) sert de laser de refroidissement. La puissance délivrée par la DFB est d'environ $\unit{60}{\milli\watt}$ et de largeur
typique $\unit{2}{\mega\hertz}$. Sa fréquence est asservie par une technique d'\emph{offset-lock}, qui sera détaillée à la section
suivante, utilisant le laser maître comme une référence de fréquence. Le waist $w$ du faisceau de refroidissement est d'une grande
importance. En effet, il a été montré dans \cite{Gattobigio2008} que pour des petits faisceaux le nombre d'atomes piégés est
proportionnel à $w^4$. Augmenter la taille des faisceaux de piégeage revient donc à augmenter la plage de capture des atomes dans le
piège, tout paramètre constant par ailleurs. De fait, si l'on veut maintenir l'intensité des laser du piège au niveau des atomes
proche de l'intensité de saturation de la transition $\ket{F = 3} \to \ket{F^{\prime} = 4}$ en augmentant leur taille, nous devons
disposer de plus de puissance. Le laser issu de la diode DFB est donc amplifié par un MOPA (Master Oscillator Power Amplifier, Sacher
TEC-400) pour obtenir jusqu'à $\unit{2}{\watt}$ de puissance lumineuse en sortie. Les faisceaux ont un waist de
$\unit{3.4}{\centi\meter}$ pour une intensité totale maximale au centre du piège d'environ
$\unit{6}{\milli\watt\cdot\centi\reciprocal\meter}$. Ce grand waist est l'originilaté majeure de notre expérience, c'est le paramètre
important pour capturer un grand nombre d'atomes par rapport à ce qui est couramment possible dans les autres expériences de
refroidissement laser. En plus des faisceaux de refroidissement, une partie de la puissance lumineuse accessible après amplification
est utilisée comme pompe et comme sonde. On dispose ainsi de lasers asservis en phase pour des expériences de type pompe-sonde.

En outre, pour maintenir constant le nombre d'atomes piégés, une autre diode DFB, de puissance $\unit{80}{\milli\watt}$ et de même
largeur que pour les faisceaux MOT, est utilisé pour repomper les atomes dans l'état $\ket{F = 3}$. Il est asservi par absorption
saturée sur le cross-over $\ket{F = 2} \to \ket{F^{\prime} = 2}/\ket{F = 2} \to \ket{F^{\prime} = 3}$ du \Rb.
  
	\paragraph{Asservissement en fréquence par \emph{offset-lock}}\label{Parag:OffsetLock}

Le premier point à maîtriser pour manipuler un nuage d'atomes froids est la fréquence des lasers. Les précédents montages mis en
place sur l'expérience asservissaient la fréquence des lasers par absorption saturée, avec donc une fréquence fixe. Pour la faire
varier et scanner pendant une phase de mesure, nous devions utiliser un modulateur acousto-optique (AOM) en configuration double
passage. Cependant, comme l'efficacité de diffraction d'un AOM dépend de la fréquence de vibration du cristal à l'intérieur, nous
sommes très vite limités dans sa gamme de fréquence accessible, au maximum de $20\Gamma$. La puissance du faisceau
diffracté change donc au cours d'un scan. En l'état, cette variation n'a pas d'influence sur une mesure de spectre de transmission.
En revanche, l'obtention d'un laser aléatoire requiert d'avoir une pompe centrée sur la transition interdite
$\ket{F = 3} \to \ket{F^{\prime} = 1}$ pour induire du gain Raman entre les deux niveaux hyperfins fondamentaux du \Rb, 
\cite{BaudouinNatPhys2013}. Dans cette expérience, la difficulté est d'avoir un laser pompe dont la puissance est constante au cours
d'un balayage de fréquence autour de la transition mentionnée précédemment. De plus, la pompe étant issue du même laser que les
faisceaux MOT, sa fréquence doit donc être décalée d'environ $35\Gamma$ par rapport à la transition du piège, voir
figure~\ref{fig:D2Lasers}. Ce décalage en fréquence n'est pas accessible par des modulateurs acousto-optiques en congiguration double
passage sans changer la puissance du laser. Pour cette raison, l'asservissement de la DFB a été modifié pour tirer parti d'un schéma
de type \emph{offset-lock} : pouvoir scanner une grande gamme de fréquence sans variation de puissance.

Nous détaillons maintenant le principe de l'asservissement de la DFB par \emph{offset-lock}. Tous les détails peuvent être retrouvés
dans
\cite{Kashanian2016}. Un schéma résumant le montage électronique est présenté sur la figure~\ref{fig:OffsetLock}. La première étape
de l'asservissement repose sur un battement entre les diodes DBR et DFB. Comme la DBR est asservie sur le cross-over
$\ket{F = 2} \to \ket{F^{\prime} = 2}/\ket{F = 2} \to \ket{F^{\prime} = 3}$ du \RbIso~et la DFB doit être asservie de sorte à être
proche de la résonance de la transition $\ket{F = 4} \to \ket{F^{\prime} = 4}$ du \Rb, la fréquence résultante du battement est
donc la différence de fréquence entre DBR et DFB, proche de $\unit{1}{\giga\hertz}$. En utilisant un mixeur de radio-fréquence,
la fréquence du battement est multipliée avec celle issue d'un oscillateur contrôlé en tension (VCO), piloté par ordinateur. On ne
garde que le signal correspondant à la différence des fréquences. En combinant un filtre passe-haut de fréquence de coupure
$\unit{300}{\mega\hertz}$ et un filtre passe-bas de fréquence de coupure $\unit{250}{\mega\hertz}$, le signal d'erreur est produit
en soustrayant la sortie des deux filtres. Le signal de rétroaction est finalement généré grâce à un contrôleur PI. La rétroaction
est ensuite envoyée à la source de courant du laser. En résumé, le choix de la fréquence du VCO est d'une importance capitale
puisqu'elle influe directement sur la fréquence finale du laser. La gamme de fréquence accessible par l'offset lock est
approximativement de  $\unit{500}{\mega\hertz}$, soit environ $80\Gamma$, ce qui est bien plus confortable que celle d'un AOM. Comme
la DFB pilote aussi bien les faisceaux MOT, qu'une sonde sur la même transition ou la pompe du laser aléatoire, le laser peut donc
faire plusieurs sauts de fréquence au cours d'un cycle expérimental. Nous devons donc caractériser la vitesse maximal d'un scan de
fréquence. Celle-ci a été mesurée en effectuant un brusque saut de fréquence et en étudiant le temps mis par le signal d'erreur pour
revenir à zéro. Nous avons mesuré qu'une centaine de micro-secondes est suffisant pour ne pas être limité par la boucle
d'asservissement dont la bande-passante est de $\unit{20}{\kilo\hertz}$. La diode DFB peut être, finalement, asservie pendant
plusieurs jours.

\begin{figure}\centering
 \input{/home/aurelien/These/Recherche/Manuscript/ExpCorr/TiKZ/OffsetLock.pgf}
  \caption{Schéma du principe d'asservissement en fréquence par \emph{offset-lock}. Le filtre radio-fréquence, délimité par un
	  rectangle en pointillé et caractérisé par sa fréquence $\omega_{\mathrm{filtre}}$, génère le signal d'erreur en faisant
	  la différence entre les sorties des détecteurs de puissance A et B. La modification du signal émis par le VCO permet le
	  changement de fréquence de la DFB, à puissance constante. PD : photodiode. Amp : amplificateur. PB : passe bas. PH :
	  passe haut.}
    \label{fig:OffsetLock}.
\end{figure}

La caractérisation précise (largeur, bruit d'intensité et de fréquence) de la DFB fournissant les faisceaux MOT sera abordée à la
section~\ref{Sec:BruitsLaser}.
      
	\paragraph{Séparateur de faisceaux fibré}\label{Parag:Fibre}

Comme mentionné précédemment, pour refroidir un nuage d'atomes, nous avons besoin de trois paires de faisceaux contra-propageants. Une
première méthode est d'utiliser des cubes séparateurs de polarisation. Il est alors possible de contrôler finement la puissance de
chaque faisceau indépendamment des autres, au prix d'avoir de longs chemins optiques à aligner régulièrement. Une autre possibilité
est d'utiliser un séparateur de faisceaux fibré, ce qui a récemment été implémenté sur notre expérience avec un séparateur de chez OZ
Optics. Les faisceaux MOT et le repompeur sont tous les deux couplés dans une même fibre à maintien de polarisation qui est ensuite
divisée en six fibres indépendantes dont les puissances sont équilibrées ($\pm 10\%$) en sortie. L'avantage de ce montage est une plus
grande stabilité de l'alignement, comme il y a moins d'optiques requises pour le MOT. La complexité du montage s'en trouve donc
fortement réduite. Les modes spatiaux des lasers à injecter ont été adaptés avec le mode d'entrée de la fibre pour en optimiser le
couplage, d'environ 50\% pour les faisceaux MOT et le repompeur. La polarisation des lasers à l'entrée de la fibre est ajustée pour la
maintenir linéaire, suivant un des ses axes, afin qu'elle soit bien stable en sortie.

Pour équilibrer les puissances des faisceaux contra-propageants, nous avons choisi deux à deux les fibres ayant des puissances de 
sortie les plus proches possibles. Pour un réglage plus fin, on peut aussi rajouter un film de polariseur directement sur un coupleur
de sortie. La polarisation circulaire ($\sigma^+$ ou $\sigma^-$) des faisceaux MOT et repompeur requise pour le piégeage est obtenue
par  un couple de lame $\lambda/2$ et $\lambda/4$ placé en aval du coupleur de sortie. Les faisceaux sont ensuite collimatés avec des
lentilles de focale $\unit{300}{\milli\meter}$ et de $\unit{10}{\centi\meter}$ de diamètre, pour des tailles typiques de
$\unit{3.4}{\centi\meter}$ pour chaque faisceau au niveau des atomes.

\begin{figure}\centering
 \input{/home/aurelien/These/Recherche/Manuscript/ExpCorr/TiKZ/RbD2.pgf}
  \caption{Schéma de la configuration laser de l'expérience. En bas~: niveaux d'énergie de la raie D2 du \Rb, présentant les 
    transitions sur lesquelles les lasers sont accordés.}
    \label{fig:D2Lasers}
\end{figure}

      \subsubsection{Contrôle des fréquences et expériences typiques}\label{Subsubsec:ContManip}
 
Le piégeage et la manipulation d'un gaz d'atomes froids requiert un contrôle fin des fréquences et des intensités des lasers
utilisés. Pour cela, comme mentionné précedemment, nous utilisons des AOMs soit en configuration simple passage soit en
configuration double passage. La première permet d'ajuster finement l'intensité d'un laser ainsi que son utilisation en tant
qu'interupteur. La seconde sert à modifier sa fréquence, et en particulier à réaliser des scans de fréquence. Ils sont tous
contrôlés par des oscillateurs radio-fréquences (VCO). Ces derniers sont pilotés par des cartes analogiques programmables
$\unit{0-10}{\volt}$ (NIPCI 6723), de pas de temps $\unit{10}{\micro\second}$ assurant le bon déroulement de la séquence
expérimentale. Tous ces dispositifs, ainsi que certains instruments de mesure utilisés dans l'expérience (caméra CCD), sont
contrôlés par une interface Matlab.

La réalisation d'expériences sur un nuage d'atomes froids nécessite un échantillon qui ne soit pas perturbé par les faisceaux du
piége ou le champ magnétique. La séquence expérimentale est donc répétée et est composée de phase de préparation et de mesure. Nous
listons maintenant les plus importantes.

Tout d'abord, les atomes sont chargés dans le MOT pendant une durée dépendante du nombre d'atomes désiré, typiquement
$\unit{30-500}{\milli\second}$. On piége ainsi jusqu'à $\power{10}{10}$ atomes. Le désaccord des faisceaux MOT est de $-3\Gamma$
par rapport à la transition $\ket{F = 3} \to \ket{F^{\prime} = 4}$ et le repompeur est à résonance sur $\ket{F = 2} \to
\ket{F^{\prime} = 3}$. Le temps de chargement peut être réduit si les atomes sont recyclés entre deux cycles, donc si le MOT n'est
pas détruit à la fin de la séquence.

S'ensuit une phase de compression. De manière générale, dans les MOT de grande taille, la densité atomique $\rho$ est limitée, en
partie, par la répulsion entre les atomes due à la diffusion multiple. Les atomes sont comme poussés vers l'extérieur du nuage par la
pression de radiation. Il en résulte une hausse de la taille du nuage ainsi qu'un chauffage des atomes \cite{Walker_1990}. Plusieurs
méthodes ont été développées pour s'affranchir de ces effets et pouvoir augmenter la densité. Par exemple, dans un MOT compressé, une
augmentation subite du gradient de champ magnétique permet de gagner environ un ordre de grandeur sur la densité, au coût d'un
chauffage du nuage~\cite{Petrich1994}. Nous avons choisi d'appliquer un piège noir, ou \emph{dark MOT} (DMOT). Ici, les atomes passent
progressivement dans un état qui ne diffuse pas la lumière du piége, $\ket{F=2}$ pour nous. Les interactions diminuent, le nuage
s'effondre sur lui-même et la densité ainsi que l'épaisseur optique augmentent au prix d'une perte du nombre d'atomes, limitée à une
quinzaine de pourcent. La compression par DMOT peut s'effectuer de deux manière différentes, soit en masquant le centre des faisceaux
du repompeur~\cite{Ketterle1993,Anderson_1994}, soit en diminuant l'intensité du repompeur par plusieurs ordres de grandeur en
quelques millisecondes~\cite{Townsend1996,Walker_1990}. Cette dernière technique est celle appliquée sur l'expérience. L'intensité du
repompeur passe à 2.5\% de sa valeure maximale pendant $\unit{35}{\milli\second}$ et le désaccord des faisceaux MOT est ramené à
$-2\Gamma$ pour augmenter l'épaisseur optique jusqu'à 160 et la densité à $\unit{\power{10}{12}}{\text{at}\cdot\meter\rpcubed}$, le
rayon rms du nuage typique étant $R \simeq \unit{1}{\milli\meter}$. L'optimisation du DMOT s'est faite uniquement sur l'épaisseur
optique, sans chercher à obtenir de compromis avec la température.

Finalement, la dernière phase est l'étape de mesure où le gradient de champ magnétique et les faisceaux du piège sont coupés. En
revanche, on peut garder allumer le repompeur pour maintenir les atomes dans l'état $\ket{F = 3}$. Pendant cette phase, les atomes
sont en expansion libre et suivent un mouvement ballistique pendant quelques milisecondes. Nous pouvons leur appliquer une sonde ou
alors les pomper pour obtenir un laser aléatoire. L'ajustement de la période d'expansion, phase de temps de vol (TOF), fait varier
l'épaisseur optique à nombre d'atomes constant.

\textcolor{red}{Rajouter une photo prise de la manip où on voit une grosse lentille, la cellule, la fibre et une bobine ?}

    \subsection{Caractérisation du nuage}\label{Subsec:CaracMOT}

Une fois le nuage préparé, plusieurs diagnostics sont disponibles pour le caractériser. Dans tous les cas, ils s'effectuent en
étudiant les propriétés de la lumière émise alors qu'il est éclairé de manière externe.
  
      \subsubsection{Détermination du temps de chargement du piège}\label{Subsubsec:Loading}

Comme nous l'avons vu, un vide poussé est nécessaire à l'obtention d'un MOT. Précisons maintenant que la qualité du vide détermine
le nombre d'atomes piégés. Il est donc important de caractériser ce nombre d'atomes en fonction de la pression résiduelle d'atomes
de rubidium à l'intérieur de la cellule. Pour cela, étudions l'évolution temporelle du nombre d'atomes.

Notre MOT est chargé à partir d'une vapeur de rubidium à l'intérieur de la cellule à vide. Les atomes sont piégés avec un flux
$\mathcal{L}$, en nombre d'atomes par seconde, proportionnel à la pression partielle de rubidium $P_{\text{Rb}}$. Un des facteurs
de perte est les collisions entre la vapeur à température ambiante (les atomes de rubidium non chargés et les gaz résiduels) avec
les atomes piégés. Les atomes à température ambiante sont susceptibles de transférer assez d'énergie à ceux refroidis pour les
expulser du piége. Définissons alors le taux de pertes $\gamma$, proportionnel à $P_{\text{Rb}}$ et $P_{\text{res}}$, la pression
résiduelle de gaz. Dans la limite où les collisions froides entre deux atomes du piéges peuvent être négligées, l'évolution
temporelle du nombre $\NbAtoms$ d'atomes s'écrit~:

\begin{equation}
 \derivee{\NbAtoms(t)}{t} = \mathcal{L} - \gamma\NbAtoms.
\end{equation}
\noindent
La solution s'écrit~:

\begin{equation}
 \NbAtoms(t) = \NbAtoms_{\inf}(1 - \e^{-\gamma{}t}),
\end{equation}
\noindent
avec la condition initiale $\NbAtoms(0) = 0$ et $\NbAtoms_{\inf} = \mathcal{L}/\gamma$ est le nombre d'atomes en régime stationnaire.
La connaissance du temps de chargement $\tau_{\text{load}} = \gamma^{-1}$ du MOT est donc une mesure directe de $P_{\text{Rb}}$. Si
$\gamma^{-1}$ est trop long, la pression partielle de rubidium est trop faible et il faut donc ré-injecter des atomes dans la cellule.
Cela est possible grâce à une source de rubidium, une goutte déposée dans un queusot, isolée de l'enceinte à vide par une valve. Une
autre possibilité est de faire désorber du rubidium des parois de la cellule à vide grâce à des diodes électro-luminescentes
ultra-violettes. Cette technique, appelée désoprtion atomique assistée par la lumière~\cite{Gozzini1993}, prend la vapeur de rubidium
libérée par les parois comme une nouvelle source d'atomes à charger dans le piège. Il a été montré dans \cite{Anderson2001,Atutov2003}
la possibilité d'utliser directement la vapeur atomique désorbée dans un piège magnéto-optique, tout en ayant de très bonnes
efficacités. Temporairement, le recours à cette stratégie permet une augmentation du nombre d'atomes piégés, à temps de chargement
fixe, et donc de l'épaisseur optique.

Le temps de chargement se mesure à partir de la collection de la fluorescence des atomes du nuage. Pour cela, on utilise une
lentille de focale $\unit{100}{\milli\meter}$ et de $\unit{50.8}{\centi\meter}$ de diamètre qui conjugue le MOT sur une photodiode.
L'axe de détection fait un angle d'environ $\unit{15}{\degree}$ avec l'axe du gradient du champ magnétique.

\textcolor{red}{Rajouter une courbe du temps de chargement, avec les bonnes unités sur l'axe des y, pour obtenir $\gamma$ et la
pression partielle de rubidium. + augmentation du nombre d'atomes avec LIAD}
    
      \subsubsection{Spectre de transmission par spectroscopie}\label{Subsubsec:SpecTrans}
  
Une fois le MOT correctement chargé, une première caractérisation est la mesure de la transmission d'une sonde de faible intensité,
et de diamètre petit devant celui du nuage, à travers les atomes. Par application de la loi de Beer-Lambert, nous définissions la
transmission $T$ par le rapport entre l'intensité transmise $I_{\text{trans}}$ et celle incidente $I_{\text{inc}}$,
$T = I_{\text{trans}} / I_{\text{inc}}$. Dans le cas d'un système passif, la mesure de $T$ en fonction du désaccord $\delta = 
\omegaL - \omega_0$ de la sonde asservie en fréquence autour de la transition $\ket{F = 3} \to \ket{F^{\prime} = 4}$ donne accès à
l'épaisseur optique à résonance $b_0$ du nuage. En supposant que les populations d'un niveau hyperfin sont équiréparties entre
l'ensemble des sous-niveaux Zeeman, la section efficace de diffusion s'écrit~:

\begin{equation}
 \sigma_{\text{sc}}(\delta) = \mathcal{C}\frac{\sigma_0}{1 + 4\delta^2/\Gamma^2},
 \label{eq:SecEffDiff}
\end{equation}
\noindent
où $\sigma_0 = \frac{3\lambda^2}{2\pi}$ est la section efficace de diffusion d'un atome à deux niveaux soumis à un laser à
résonance de longueur d'onde $\lambda$ et $\mathcal{C} = 3/7$ le coefficient de Clebsh-Gordan moyenné sur l'ensemble des
sous-niveaux Zeeman de la transition étudiée. On obtient, au final, l'expression de la transmission $T_{\text{at}}$ à travers les
atomes~:

\begin{equation}
 T_{\text{at}}(\delta) = \exp\left( -\frac{b_0}{1 + 4\delta^2/\Gamma^2} \right).
 \label{eq:Trans}
\end{equation}

Expérimentalement, trois quantités doivent être mesurées pour accéder à $T$ : l'intensité en absence de sonde et d'atomes
($I_{\text{BG}}$), l'intensité sans ($I_{\text{sans}}$) et avec ($I_{\text{avec}}$) atomes. Au final, nous déduisons~:

\begin{equation}
 T = \frac{I_{\text{avec}} - I_{\text{BG}}}{I_{\text{sans}} - I_{\text{BG}}}.
\end{equation}
\noindent
Cette technique a l'avantage de mesurer la transmission sans avoir à déterminer l'intensité de la sonde. On s'affrachit donc de
ses fluctuations en fonction des conditions expérimentales (réponse de l'AOM, polarisation, ...). L'intensité de la sonde doit,
cependant, être faible devant l'intensité de saturation de la transition
$I_{\text{sat}} = \unit{1.6}{\milli\watt\cdot\centi\meter\rpsquared}$ pour s'assurer d'une réponse linéaire du nuage avec
l'intensité du laser. La sonde utilisée a un waist de $\unit{260}{\micro\meter}$ au niveau des atomes, de diamètre typique
$\unit{1}{\milli\meter}$ et est détectée sur une photodiode (\textcolor{red}{caractéristique de la photodiode}). Une mesure typique de
spectre de transmission est présentée sur la figure~\ref{fig:Sonde}.

\begin{figure}\centering
 \input{/home/aurelien/These/Recherche/Manuscript/ExpCorr/TiKZ/Sonde.pgf}
  \caption{Mesures d'un spectre de transmission de la sonde en fonction du désaccord par rapport à la résonance atomique. Un 
    ajustement par la formule\eqref{eq:Trans} donne accès à $b_0$. En haut, nous présentons le schéma de la configuration 
    expérimentale.}
    \label{fig:Sonde}
\end{figure}

Une fois la mesure faite, un ajustement des données par l'équation~\eqref{eq:Trans} permet une bonne estimation de $b_0$, l'origine
des fréquences étant peu importante lors de ce type de diagnostic \footnote{Ce qui ne serait pas posssible si la transmission est
mesurée point par point, avec une sonde de fréquence fixe. Dans ce cas là, la calibration du VCO contrôlant la fréquence de la 
sonde est très importante pour éviter tout décalage rédibitoire lors de mesures ultérieures.} où elle peut être laissée comme
paramètre libre. Précisons que nous tenons compte lors de l'ajustement de la transition située à $-20\Gamma$ pour corriger une
asymétrie rouge/bleu observée dans les spectres. En revanche, il faut bien s'assurer que le laser passe par le centre du nuage.
L'expression~\eqref{eq:Trans} n'est en fait valable que pour un laser parfait, avec une largeur spectrale infiniment fine. Or, la
sonde utilisée a une largeur typique de $\unit{2}{\mega\hertz}$. Une convolution entre $T$ mesurée et le  spectre du laser doit être
faite pour calculer correctement la transmission. Nous avons vérifié que cette correction a un effet néglibeable sur les épaisseurs
optiques obtenues par ajustement avec $T_{\text{at}}$.

Mentionnons enfin que l'on peut aussi mesurer la transmission d'une sonde avec un milieu actif, cette fois-ci. Il sera alors
possible de mettre en évidence une éventuelle amplification de la sonde à une fréquence bien déterminée. Ce type de mesure sera
faite pour déterminer la longueur de gain à l'intérieur du nuage.

      \subsubsection{Imagerie d'absorption}\label{Subsubsec:ImAbs}
  
Un spectre de transmission donne accès à l'épaisseur optique, mais ne nous renseigne pas sur le nombre d'atomes du nuage ni sur sa
taille. Pour cela, nous utilisons une technique d'imagerie qui consiste à envoyer une sonde collimatée de grande taille sur le nuage
pour imager son ombre. On réalise donc une image globale de la transmission des atomes quelque soit leur position dans le MOT.
L'obtention de cette image permet la mesure de la taille transverse du système. Connaissant le désaccord de la sonde, on déduit de
l'image de la transmission une carte de l'épaisseur optique. L'intensité transmise est, comme nous l'avons vu en appliquant la loi de
Beer-Lambert~:

\begin{equation}
 I_{\text{trans}}(x, y, z) = I_{\text{inc}}(x, y, z)\exp\left( -\sigma_{\text{sc}}(\delta) \int_{-\inf}^{z} \mathrm{d}z^{\prime}\,
	n(x, y, z^{\prime})\right),
	 \label{eq:BeerLamInt}
\end{equation}
\noindent
où $\rho$ est la densité atomique, $z^{\prime}$ est la direction de propagation du faisceau d'imagerie et
$\sigma_{\text{sc}}(\delta)$ est définie par l'équation~\eqref{eq:SecEffDiff}. L'épaisseur optique s'écrit de manière générale~:

\begin{equation}
 b(\delta) = \sigma_{\text{sc}}(\delta)\int_{-\inf}^{z} \mathrm{d}z^{\prime}\,n(x, y, z^{\prime}).
  \label{eq:EpOptInt}
\end{equation}

Supposons maintenant que le nuage a une distribution spatiale gaussienne de largeur rms $\sigma_j$ selon la direction $j$. Nous
obtenons donc le nombre d'atomes dans le MOT, en faisant appraître l'épaisseur optique du nuage à la fréquence du laser mesurée
selon l'axe $z$ passant par le centre du nuage~:

\begin{equation}
 \NbAtoms = 2\pi\sigma_{x}\sigma_{y}\frac{b(\delta)}{\sigma_{\text{sc}}(\delta)}.
\end{equation}
\noindent
Nous en déduisons la densité $\rho_0$ au centre du nuage~:

\begin{equation}
 n_0 = \frac{\NbAtoms}{(2\pi)^{3/2}\sigma_{x}\sigma_{y}\sigma_{z}}.
\end{equation}
\noindent
La géométrie du nuage est supposée quasi-sphérique, d'où $\sigma_{z} = (\sigma_{x} + \sigma_{y})/2$. La figure~\ref{fig:Compb0} montre
la comparaison entre les épaisseurs optiques à résonance obtenues par imagerie d'absorption et \emph{via} un spectre de transmission.

\begin{figure}\centering
 \includegraphics[scale=1]{/home/aurelien/These/Recherche/Manuscript/ExpCorr/Images/EpOP_TransVsIm.eps}
  \caption{Comparaison entre les épaisseurs optiques mesurées grâce à un spectre de transmission et par l'imagerie d'absorption. La
    ligne pointillée représente l'identité.}
      \label{fig:Compb0}
\end{figure}

Comme pour le spectre de transmission, l'imagerie par absorption requiert trois images pour ne pas être limitée par les fluctuations
d'intensité de la sonde. La taille du nuage varie d'une centaine de micromètre au milimètre. Un doublet de lentilles, assurant un
\textcolor{red}{grandissement}, est utilisé pour imager le nuage sur une caméra CCD (modèle Pointgray GRAS-20S4M-C) reliée à un
ordinateur. Même si le temps d'exposition est court (une centaine de microseconde), l'utitilisation de l'imagerie d'absorption peut
être contraignante. En effet, la prise de trois images est longue ($\unit{200}{\milli\second}$) et détruit le nuage.
  
L'imagerie d'absorption peut aussi servir de thermomètre par application d'un temps de vol, période où le nuage est en expansion
libre sans faisceaux MOT (mais en présence de repompeur pour maintenir la population dans l'état $\ket{F = 3}$) ni gradient de
champ magnétique. Au cours de cette phase, le nuage n'est donc soumis qu'à son propre poids sous l'effet de la gravité terrestre.
L'équation horaire du mouvement des atomes est donc celle bien connue de la chute libre. Supposons que le nuage s'étend de manière
homogène et que vitesse et position à un instant $t$ sont décorrélées. Malgré la nature quantique des atomes, le MOT peut être
décrit en excellente approximation par un gaz thermique. Celui-ci a une distribution maxwellienne des vitesses caractérisée par sa
vitesse quadratique moyenne $\braket{v^{2}} = \frac{\kB\temp}{m}$, où $\kB$ est la constante de Boltzmann, $\temp$ la
température du nuage et $m$ la masse d'un atome de \Rb. Dans ce cas, en manipulant l'équation du mouvement et en négligeant l'effet de
la gravité, la taille transverse rms ($j = x, y$) du nuage suit la loi horaire~:

\begin{equation}
 \sigma_{j}{}^2(t) = \sigma_{0}{}^2 + \frac{\kB\temp}{m}t^2.
 \label{eq:TOF}
\end{equation}
\noindent
La prise de plusieurs images à différents temps de vol pour mesurer les tailles correspondantes du nuage sont donc une estimation
de la température des atomes. Dans notre cas, nous obtenons $\temp \sim \unit{200}{\micro\kelvin}$, comme montré sur la
figure~\ref{fig:TOF}.

\begin{figure}\centering
 \input{/home/aurelien/These/Recherche/Manuscript/ExpCorr/TiKZ/AbsIm.pgf}
  \caption{Mesure de la température par temps de vol, pour les deux directions $x$ (en rouge) et $y$ (en nuance de gris). L'ajustement 
    des données par la formule~\eqref{eq:TOF} donne $\temp_x = \unit{244}{\micro\kelvin}$ et $\temp_y = \unit{230}{\micro\kelvin}$,
    respectivement. Les barres d'erreur sont obtenues en moyennant les tailles transverses sur cinq images. En haut, nous présentons
    la configuration expérimentale, où le faisceau d'imagerie est couplé dans une fibre mono-mode.}
      \label{fig:TOF}
\end{figure}

Mentionnons que la mesure de $b_0$, par imagerie ou par transmission, permet aussi de déduire la température du nuage. En effet,
on montre que, pour un nuage gaussien à trois dimension~:

\begin{equation}
 b_0 = \mathcal{C}\frac{3\NbAtoms}{(k\sigma)^2},
 \label{eq:bo_vs_N}
\end{equation}
\noindent
où $k = 2\pi/\lambda$ est le vecteur d'onde de la sonde à résonance et $\sigma = \sqrt{\sigma_{x}\sigma_{y}}$ est la moyenne
géométrique de la taille du nuage. En combinant les équations~\eqref{eq:TOF} et~\eqref{eq:bo_vs_N}, et en supposant les tailles
suivant $x$ et $y$ égales~:

\begin{equation}
 b_0(t) = \mathcal{C}\frac{3\NbAtoms}{(k\sigma)^2}\frac{1}{1 + \frac{\kB\temp}{m\sigma^2}t^2}.
\end{equation}
\noindent
Cette technique nécessite cependant une bonne connaissance de la taille du nuage pour donner une estimation correcte de la 
température.

      \subsubsection{Rayonnement de fluorescence}\label{Subsubsec:Fluo}
    
Quand le nuage est éclairé par les faisceaux pompes, la fluorescence émise par les atomes peut servir à caractériser la présence de
gain. L'observation d'une augmentation à une fréquence donnée du laser pompe peut réveler la présence d'un laser aléatoire
\cite{BaudouinNatPhys2013}. On collecte donc le rayonnement émis par le nuage dans un angle solide de $\power{10}{-2}\,\text{str}$
puis on mesure l'intensité du rayonnement sur un photomultipicateur de gain et bande-passante réglables. L'axe de détection fait
un angle d'environ $\unit{40}{\degree}$ avec l'axe des pompes du laser aléatoire. En tenant compte de la symétrie sphérique du
système, nous ferons l'hypothèse dans le suite de cette thèse que l'intensitée détectée est proportionnelle à l'intensité totale de
la fluorescence émise dans tout l'angle solide.

Le couplage de photons de fluorescence dans une fibre mono-mode, et leur détection sur
des photodiodes à avalanche capable de mesurer des photons uniques, rend possible la mesure des corrélations d'intensité de la lumière
diffusée.

  \section{Caractérisation d'un laser aléatoire à atomes froids par l'étude des corrélations d'intensité}\label{Sec:CARL}
  
    \subsection{Combiner du gain et de la diffusion dans un gaz d'atomes froids}\label{Subsec:GainDiffCA}
    
Expression du seuil dans les atomes froids qu'en terme de polarisabilité. Schéma du gain Rama hyperfin.

    \subsection{Observation expérimentale}\label{Subsec:ExpRL}
    
Mesure du laser aléatoire à la maison. \cite{BaudouinNatPhys2013,Baudouin2014a}

    \subsection{Vers une détection directe}\label{Subsec:ObsDirRL}
    
Comment avoir une observation directe de l'émission de laser aléatoire ?
